Observational Analysis of Lyman-alpha Emission in Equivalent Magnitude Solar Flares

The chromospheric Lyman-alpha line of neutral hydrogen (Ly$\alpha$; 1216 \r{A}) is the most intense emission line in the solar spectrum, yet until recently observations of flare-related Ly$\alpha$ emission have been scarce. Here, we examine the relationship between nonthermal electrons accelerated during the impulsive phase of three M3 flares that were co-observed by RHESSI, GOES, and SDO, and the corresponding response of the chromosphere in Ly$\alpha$. Despite having identical X-ray magnitudes, these flares show significantly different Ly$\alpha$ responses. The peak Ly$\alpha$ enhancements above quiescent background for these flares were 1.5%, 3.3%, and 6.4%. However, the predicted Ly$\alpha$ enhancements from FISM2 were consistently <2.5%. By comparing the properties of the nonthermal electrons derived from spectral analysis of hard X-ray observations, flares with a harder spectral index were found to produce a greater Ly$\alpha$ enhancement. The percentage of nonthermal energy radiated by the Ly$\alpha$ line during the impulsive phase was found to range from 2.0-7.9%. Comparatively, the radiative losses in He II (304 \r{A}) were found to range from 0.6-1.4% of the nonthermal energy while displaying enhancements above the background of 7.3-10.8%. FISM2 was also found to underestimate the level of He II emission in two out of the three flares. These results may have implications for space weather studies and modelling the response of the terrestrial atmosphere to changes in the solar irradiance, and will guide the interpretation of flare-related Ly$\alpha$ observations that will become available during Solar Cycle 25.

==> commands.tex <==
% Please use \newcommand not \def to avoid
% overwriting existing commands. Example:
%\newcommand{\pcm}{\,cm$^{-2}$}	% per cm-squared
\newcommand\todo[1]{\textcolor{red}{\textbf{#1}}}
\newcommand{\kepler}{{\it Kepler}}
\newcommand{\corot}{{\it CoRoT}}
\newcommand{\tess}{{\it TESS}}
\newcommand{\plato}{{\it PLATO}}
\newcommand{\gaia}{{\it Gaia}}
\newcommand{\JWST}{{\it JWST}}
\newcommand{\NGTS}{NGTS}
\newcommand{\TESS}{{\it TESS}}
\newcommand{\gpe}{{GP-EBOP}}
\newcommand{\LSO}{La Silla Observatory}
\newcommand{\PAR}{Paranal Observatory}
\newcommand{\etop}{\emph{top}}
\newcommand{\emid}{\emph{middle}}
\newcommand{\ebot}{\emph{bottom}}
\newcommand{\eleft}{\emph{left}}
\newcommand{\eright}{\emph{right}}
\newcommand{\eTop}{\emph{Top}}
\newcommand{\eMid}{\emph{Middle}}
\newcommand{\eBot}{\emph{Bottom}}
\newcommand{\eLeft}{\emph{Left}}
\newcommand{\eRight}{\emph{Right}}
\newcommand{\btgc}[1]{\textcolor{blue}{[BTG: #1]}}
\newcommand{\jsj}[1]{\textcolor{blue}{[JSJ: #1]}}
% UNITS
\newcommand{\kms}{km\,s$^{-1}$}
\newcommand{\ms}{m\,s$^{-1}$}
\newcommand{\masy}{mas\,y$^{-1}$}
\newcommand{\mpl}{\mbox{M$_{P}$}}
\newcommand{\rpl}{\mbox{R$_{P}$}}
\newcommand{\rhopl}{\mbox{$\rho_{P}$}}
\newcommand{\mstar}{\mbox{M$_{*}$}}
\newcommand{\rstar}{\mbox{R$_{*}$}}
\newcommand{\rhostar}{\mbox{$\rho_{*}$}}
\newcommand{\mjup}{\mbox{M$_{J}$}}
\newcommand{\rjup}{\mbox{R$_{J}$}}
\newcommand{\rhojup}{\mbox{$\rho_{J}$}}
\newcommand{\mearth}{\mbox{M$_{\oplus}$}}
\newcommand{\rearth}{\mbox{R$_{\oplus}$}}
\newcommand{\msun}{\mbox{M$_{\odot}$}}
\newcommand{\rsun}{\mbox{R$_{\odot}$}}
\newcommand{\gccc}{g\,cm$^{-3}$}
\newcommand{\ergscm}{erg\,s$^{-1}$cm$^{-2}$}
\newcommand{\teff}{$T_{\rm eff}$}
\newcommand{\feh}{\mbox{[Fe/H]}}
\newcommand{\vsini}{\mbox{$v\sin i$}}
\newcommand{\logg}{$\log g$}
\newcommand{\tc}{$T_C$}
\newcommand{\rprs}{\mbox{R$_{P}/$R$_{*}$}}
\newcommand{\lya}{Ly$\rm \alpha$}
\newcommand{\ergs}{erg\,s$\rm ^{-1}$}
\newcommand{\ec}{E$\rm _{c}$}
%Maths stuff
\newcommand{\lnL}{\mbox{$\ln\mathcal{L}$}}
\newcommand{\scin}{scintillation}
\newcommand{\sigY}{$\sigma_{\scriptscriptstyle \text{Y}}$}
\newcommand{\sigYmath}{\sigma_{\scriptscriptstyle \text{Y}}}
\newcommand{\Cy}{$C_{\scriptscriptstyle \text{Y}}$}
\newcommand{\CyMath}{C_{\scriptscriptstyle \text{Y}}}
\newcommand{\Gmag}{$G_{\text{mag}}$}
